Naamapadam: A Large-Scale Named Entity Annotated Data for Indic Languages

We present, Naamapadam, the largest publicly available Named Entity Recognition (NER) dataset for the 11 major Indian languages from two language families. The dataset contains more than 400k sentences annotated with a total of at least 100k entities from three standard entity categories (Person, Location, and, Organization) for 9 out of the 11 languages. The training dataset has been automatically created from the Samanantar parallel corpus by projecting automatically tagged entities from an English sentence to the corresponding Indian language translation. We also create manually annotated testsets for 9 languages. We demonstrate the utility of the obtained dataset on the Naamapadam-test dataset. We also release IndicNER, a multilingual IndicBERT model fine-tuned on Naamapadam training set. IndicNER achieves an F1 score of more than $80$ for $7$ out of $9$ test languages. The dataset and models are available under open-source licences at https://ai4bharat.iitm.ac.in/naamapadam.

==> backup.tex <==
% \begin{table*}[ht]
% \centering
% \begin{tabular}{|c||c||c|c|c|c|}
% \hline
% Train data & Test data & LOC & ORG & PER & Overall \\
% \hline
% \hline
% Mined (filtered) & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.83 & 0.68 & 0.81 & \textbf{0.78} \\
% ~ & FIRE & 0.73 & 0.28 & 0.51 & 0.60 \\
% ~ & WikiAnn & 0.70 & 0.40 & 0.64 & 0.60 \\
% \hline
% FIRE & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.69 & 0.20 & 0.54 & 0.51 \\
% ~ & FIRE & 0.770 & 0.333 & 0.665 & \textbf{0.698} \\
% ~ & WikiAnn & 0.62 & 0.15 & 0.26 & 0.41 \\
% \hline
% WikiAnn & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.60 & 0.22 & 0.52 & 0.44 \\
% ~ & FIRE & 0.54 & 0.12 & 0.31 & 0.39 \\
% ~ & WikiAnn & 0.89 & 0.86 & 0.84 & \textbf{0.87} \\
% \hline
% \end{tabular}
% \caption{F1 score for three models on the three testsets after filtering (Hindi).}
% \label{table:mbert_cross_hindi}
% \end{table*}

\begin{comment}
\subsection{Training a multilingual model}
NLP systems rely on annotated data to learn, these models are generally trained on a single language, and its scope is limited to that language. Since collecting data for every language is not easy, cross-lingual language understanding and low resource cross-language knowledge transfer techniques are used and shown to be effective \cite{conneau2018xnli}. 
It is observed that low resource languages can benefit enormously from multilingual fine-tuning due to the similarity of the languages belonging to a single-family \cite{baumann-2019-multilingual} \cite{dhamecha2021role}. Multilingual fine-tuning is also slightly worse when there is a large pool of languages used without considering language similarity and relatedness \cite{tsai2019small}. In these cases, another level of fine-tuning on a specific language is effective.
Since we are already dealing with low resource languages, we train an mBERT model with the mined corpus for all eleven languages combined. 
This model is trained on a total of 6 million sentences from all eleven languages. The F1 scores on the eleven mined testsets are present in table \ref{table:BaselineF1}. Clearly, this model performs best on average.\\
Note that the multilingual model trained on the datasets created usind the awesome align projections performed the best.
\end{comment}

% Quite clearly, the mined model has gained F1 score in its own test set. But the model's performance on FIRE and WikiAnn test set does not seem to be affected. This can be due to two reasons, one being that the filtered test set itself is now better and hence improving the score, secondly, the other test sets domains are different enough to not affect the score. Another interesting thing we see is that the score of all three models on the mined (filtered) test set has gone up. This makes us believe that the filtered data does in fact have less errors.

% \begin{table*}[t]
% \centering
% \begin{tabular}{|c||c||c|c|c|c|}
% \hline
% Train data & Test data & LOC & ORG & PER & Overall \\
% \hline
% \hline
% Mined (filtered) & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.776 & 0.655 & 0.791 & 0.756 \\
% ~ & FIRE & 0.53 & 0.13 & 0.30 & 0.447 \\
% ~ & WikiAnn & 0.203 & 0.53 & 0.47 & 0.47 \\
% \hline
% FIRE & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.53 & 0.23 & 0.38 & 0.40 \\
% ~ & FIRE & 0.674 & 0.266 & 0.432 & 0.577 \\
% ~ & WikiAnn & 0.087 & 0.387 & 0.303 & 0.298 \\
% \hline
% WikiAnn & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.468 & 0.231 & 0.419 & 0.387 \\
% ~ & FIRE & 0.367 & 0.145 & 0.116 & 0.280 \\
% ~ & WikiAnn & 0.902 & 0.949 & 0.915 & 0.928 \\
% \hline
% \end{tabular}
% \caption{F1 score for three models on the three test sets after filtering (Bengali).}
% \label{table:mbert_cross_bengali}
% \end{table*}

% Now that the results start to look promising, we expand our language horizon to include Bengali and Marathi, at least one of us understand these languages and can validate the mined data and results. We also have FIRE dataset for Bengali and IIT-B dataset for Marathi. We train a model on each of these datasets and test across all three test sets. The results are given in table \ref{table:mbert_cross_bengali} and \ref{table:mbert_cross_marathi}, respectively. We can see from the F1 scores that the ``ORG" tag suffers the most while cross-testing. The previous observation of the model trained on mined data having the highest average score holds true here as well. 


% \begin{table*}[t]
% \centering
% \begin{tabular}{|c||c||c|c|c|c|}
% \hline
% Train data & Test data & LOC & ORG & PER & Overall \\
% \hline
% \hline
% Mined (filtered) & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.755 & 0.654 & 0.804 & 0.751 \\
% ~ & IITB & 0.42 & 0.13 & 0.232 & 0.376 \\
% ~ & WikiAnn & 0.606 & 0.15 & 0.367 & 0.47 \\
% \hline
% IITB & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.50 & 0.168 & 0.527 & 0.336 \\
% ~ & IITB & 0.783 & 0.360 & 0.579 & 0.720 \\
% ~ & WikiAnn & 0.572 & 0.215 & 0.344 & 0.473 \\
% \hline
% WikiAnn & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.509 & 0.225 & 0.605 & 0.481 \\
% ~ & IITB & 0.509 & 0.186 & 0.313 & 0.453 \\
% ~ & WikiAnn & 0.869 & 0.7492 & 0.844 & 0.8429 \\
% \hline
% \end{tabular}
% \caption{F1 score for three models on the three test sets after filtering (Marathi).}
% \label{table:mbert_cross_marathi}
% \end{table*}

% To explain this gap in performance across datasets, we again look into the example sentences from the test sets and compare the given label versus the predicted output. Some examples and observations are given in the appendix. Moreover, the role of filtering is not exactly visible, some more analysis is done, overall result ...

\begin{comment}
\subsubsection{Fine-tuning models trained on mined data}
As mentioned previously, the model trained on a particular dataset does best on its own test set, and there is a significant drop when predictions are evaluated for other datasets. Hence, we speculate that the datasets might have some domain-specific bias. So we now experiment with further fine-tuning our mined mBERT model using a particular dataset (FIRE and WikiAnn) and check the results. We will refer to these models as ``Mined tuned on FIRE" and ``Mined tuned on Wiki" respectively. While tuning, we start with relatively smaller learning rate (1e-5) so that the learnings from the previous (mined) data is not entirely overwritten. 
The results for this are given in \ref{table:fine_tuning_with_AI4B_pretrain}.
\end{comment}
% \begin{table*}[]
% \centering
% \begin{tabular}{|c||c||c|c|c|c|}
% \hline
% Model & Test data & LOC & ORG & PER & Overall \\
% \hline
% \hline
% Mined tuned on FIRE & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.821 & 0.639 & 0.784 & 0.753 \\
% ~ & FIRE & 0.7915 & 0.3761 & 0.644 & 0.70 \\
% ~ & WikiAnn & 0.706 & 0.35 & 0.62 & 0.596 \\
% \hline
% Mined tuned on Wiki & & & & &\\
% \hline
% ~ & Mined (filtered) & 0.803 & 0.602 & 0.780 & 0.727 \\
% ~ & FIRE & 0.708 & 0.221 & 0.524 & 0.578 \\
% ~ & WikiAnn & 0.907 & 0.888 & 0.852 & 0.891 \\
% \hline
% \end{tabular}
% \caption{F1 score for the further fine-tuned models on the three testsets (Hindi).}
% \label{table:mbert_tuned_hindi}
% \end{table*}

We get visible gains for most languages when we use the mined model as the starting point and then fine-tune it to a specific dataset. One key feature to point out here is that ``Mined tuned on Wiki" models are performing consistently better than when trained only on WikiAnn data. Also, these models tend to retain a significant amount of their base training, and hence the Mined test set scores are also on par.


\subsection{Using the human annotated testset}
The mined testset used till now is the one which was algorithmically mined using the projection technique discussed at the beginning. We also created a small human-annotated testset (40-50 sentences for each language we could) to get a better understanding of our model as well as mined dataset. The mined multilingual model scores on the respective datasets are given in \ref{table:MultiTest}.
In this paper we also propose a larger human annotated testset for bengali, hindi, malayalam, marathi and kannada. The scores of our model on this testset is also given in table \ref{table:big_human_all_dataset}.


% \begin{table*}[]
% \centering
% \begin{tabular}{|l|rrrr|rrrr|}
% \hline
%  & \multicolumn{4}{c|}{\textbf{AI4B-multilingual (Giza++)}} & \multicolumn{4}{c|}{\textbf{Ai4B-multilingual (Awesome Align)}} \\ \hline
% Lang & \multicolumn{1}{l|}{LOC} & \multicolumn{1}{l|}{ORG} & \multicolumn{1}{l|}{PER} & \multicolumn{1}{l|}{Overall F1} & \multicolumn{1}{l|}{LOC} & \multicolumn{1}{l|}{ORG} & \multicolumn{1}{l|}{PER} & \multicolumn{1}{l|}{Overall F1} \\ \hline
% bn & \multicolumn{1}{r|}{75.35} & \multicolumn{1}{r|}{73.60} & \multicolumn{1}{r|}{84.07} & 79.06 & \multicolumn{1}{r|}{77.08} & \multicolumn{1}{r|}{72.98} & \multicolumn{1}{r|}{84.72} & \textbf{79.75} \\ \hline
% hi & \multicolumn{1}{r|}{81.90} & \multicolumn{1}{r|}{73.51} & \multicolumn{1}{r|}{87.52} & 80.86 & \multicolumn{1}{r|}{82.41} & \multicolumn{1}{r|}{74.63} & \multicolumn{1}{r|}{89.99} & \textbf{82.33} \\ \hline
% kn & \multicolumn{1}{r|}{72.22} & \multicolumn{1}{r|}{67.61} & \multicolumn{1}{r|}{81.99} & 75.67 & \multicolumn{1}{r|}{76.46} & \multicolumn{1}{r|}{73.46} & \multicolumn{1}{r|}{85.66} & \textbf{80.01} \\ \hline
% ml & \multicolumn{1}{r|}{76.55} & \multicolumn{1}{r|}{55.78} & \multicolumn{1}{r|}{79.03} & 73.62 & \multicolumn{1}{r|}{82.90} & \multicolumn{1}{r|}{61.59} & \multicolumn{1}{r|}{87.02} & \textbf{80.73} \\ \hline
% mr & \multicolumn{1}{r|}{76.04} & \multicolumn{1}{r|}{57.25} & \multicolumn{1}{r|}{83.78} & 74.92 & \multicolumn{1}{r|}{82.64} & \multicolumn{1}{r|}{65.89} & \multicolumn{1}{r|}{87.05} & \textbf{80.51} \\ \hline
%  & \multicolumn{4}{c|}{\textbf{Fire-Models}} & \multicolumn{4}{c|}{\textbf{Wiki-Models}} \\ \hline
%  & \multicolumn{1}{l|}{LOC} & \multicolumn{1}{l|}{ORG} & \multicolumn{1}{l|}{PER} & \multicolumn{1}{l|}{Overall F1} & \multicolumn{1}{l|}{LOC} & \multicolumn{1}{l|}{ORG} & \multicolumn{1}{l|}{PER} & \multicolumn{1}{l|}{Overall F1} \\ \hline
% bn & \multicolumn{1}{r|}{64.01} & \multicolumn{1}{r|}{24.29} & \multicolumn{1}{r|}{37.19} & 43.30 & \multicolumn{1}{r|}{50.23} & \multicolumn{1}{r|}{26.05} & \multicolumn{1}{r|}{48.10} & 43.33 \\ \hline
% hi & \multicolumn{1}{r|}{72.51} & \multicolumn{1}{r|}{31.89} & \multicolumn{1}{r|}{59.93} & 58.09 & \multicolumn{1}{r|}{63.19} & \multicolumn{1}{r|}{29.09} & \multicolumn{1}{r|}{61.05} & 50.35 \\ \hline
% kn & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{r|}{54.66} & \multicolumn{1}{r|}{31.29} & \multicolumn{1}{r|}{65.15} & 54.37 \\ \hline
% ml & \multicolumn{1}{r|}{72.06} & \multicolumn{1}{r|}{34.06} & \multicolumn{1}{r|}{59.88} & 58.91 & \multicolumn{1}{r|}{66.06} & \multicolumn{1}{r|}{29.46} & \multicolumn{1}{r|}{69.03} & 59.42 \\ \hline
% mr & \multicolumn{1}{r|}{64.24} & \multicolumn{1}{r|}{23.77} & \multicolumn{1}{r|}{63.98} & 56.59 & \multicolumn{1}{r|}{63.02} & \multicolumn{1}{r|}{30.00} & \multicolumn{1}{r|}{72.68} & 59.66 \\ \hline
%  & \multicolumn{4}{c|}{\textbf{SemEval-Models}} & \multicolumn{4}{c|}{\textbf{CFILT}} \\ \hline
%  & \multicolumn{1}{l|}{LOC} & \multicolumn{1}{l|}{ORG} & \multicolumn{1}{l|}{PER} & \multicolumn{1}{l|}{Overall F1} & \multicolumn{1}{l|}{LOC} & \multicolumn{1}{l|}{ORG} & \multicolumn{1}{l|}{PER} & \multicolumn{1}{l|}{Overall F1} \\ \hline
% bn & \multicolumn{1}{r|}{34.87} & \multicolumn{1}{r|}{28.18} & \multicolumn{1}{r|}{25.60} & 29.43 & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} \\ \hline
% hi & \multicolumn{1}{r|}{47.51} & \multicolumn{1}{r|}{30.15} & \multicolumn{1}{r|}{59.21} & 45.69 & \multicolumn{1}{r|}{82.54} & \multicolumn{1}{r|}{71.49} & \multicolumn{1}{r|}{78.95} & 78.03 \\ \hline
% kn & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} \\ \hline
% ml & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} \\ \hline
% mr & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} & \multicolumn{1}{l|}{-} \\ \hline
% \end{tabular}
% \caption{Results of each datasets models on large human annotated test sets.}
% \label{table:big_human_all_dataset}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


\section{Overall Results and Discussions}



\begin{table*}[]
\begin{tabular}{|l|rr|rr|ll|}
\hline
\textbf{Test-sets} & \multicolumn{2}{l|}{\textbf{AI4B awesome Test-set}} & \multicolumn{2}{l|}{\textbf{Wiki Testset}} & \multicolumn{2}{l|}{\textbf{Fire Test-set}} \\ \hline
Models & \multicolumn{1}{l|}{AI4B (awesome)} & \multicolumn{1}{l|}{WikiAnn} & \multicolumn{1}{l|}{AI4B(Awesome)} & \multicolumn{1}{l|}{WikiAnn} & \multicolumn{1}{l|}{AI4B (Awesome)} & WikiAnn \\ \hline
as & \multicolumn{1}{r|}{62.50} & 6.74 & \multicolumn{1}{r|}{44.12} & 84.30 & \multicolumn{1}{l|}{} & \\ \hline
bn & \multicolumn{1}{r|}{80.16} & 42.40 & \multicolumn{1}{r|}{52.02} & 92.87 & \multicolumn{1}{r|}{48.46} & \multicolumn{1}{r|}{28.09} \\ \hline
gu & \multicolumn{1}{r|}{77.80} & 42.79 & \multicolumn{1}{r|}{51.93} & 85.57 & \multicolumn{1}{l|}{} & \\ \hline
hi & \multicolumn{1}{r|}{79.59} & \multicolumn{1}{r|}{45.99} & \multicolumn{1}{r|}{62.20} & 87.56 & \multicolumn{1}{r|}{60.20} & \multicolumn{1}{r|}{39.36} \\ \hline
kn & \multicolumn{1}{r|}{79.02} & 50.73 & \multicolumn{1}{r|}{64.43} & 76.95 & \multicolumn{1}{l|}{} & \\ \hline
ml & \multicolumn{1}{r|}{79.96} & 51.85 & \multicolumn{1}{r|}{64.09} & 83.71 & \multicolumn{1}{r|}{61.43} & \multicolumn{1}{r|}{52.78} \\ \hline
mr & \multicolumn{1}{r|}{79.42} & 53.82 & \multicolumn{1}{r|}{57.94} & 84.29 & \multicolumn{1}{r|}{59.51} & \multicolumn{1}{r|}{45.35} \\ \hline
or & \multicolumn{1}{r|}{27.05} & 03.77 & \multicolumn{1}{r|}{01.07} & 16.81 & \multicolumn{1}{l|}{} & \\ \hline
pa & \multicolumn{1}{r|}{74.88} & 32.86 & \multicolumn{1}{r|}{40.78} & 59.65 & \multicolumn{1}{l|}{} & \\ \hline
ta & \multicolumn{1}{r|}{76.80} & 46.26 & \multicolumn{1}{r|}{42.45} & 77.64 & \multicolumn{1}{r|}{60.23} & \multicolumn{1}{r|}{40.02} \\ \hline
te & \multicolumn{1}{r|}{78.37} & 46.66 & \multicolumn{1}{r|}{57.85} & 80.00 & \multicolumn{1}{l|}{} & \\ \hline
\end{tabular}
\caption{Cross domain testing of mined and wiki models.}
\label{table:crosstest}
\end{table*}





\subsection{Zero Shot and Teacher-Student}
Zero shot and teacher student models are a very popular way to create models which can predict named entities for languages which do not have an NER data set of their own. These techniques were tried on multiple datasets of available Indian languages. The scores obtained through this method can be seen in table \ref{table:ai4bharatTestSetResults} and the scores obtained on the same data set using a model trained on our mined data can be seen as well. Our model outperforms these approaches across the board and is a straight up upgrade to these existing approaches (on all testsets).

\subsection{Foreign Data sets}
Most of the existing labelled data sets such as WikiAnn boast high scores on their in domain test sets. However the performance of these models vastly reduces when using an out of domain test set. This shows a heavy bias in the model that's been trained. But the model trained on our mined data is far more generic getting competitive scores even on out of domain test sets while maintaining the highest scores on its in-domain test sets. \\
These can be observed the best by comparing the WikiAnn models to our mined models and using the Fire test set. While the wiki model scores very high on its Wiki test set, its scores on our mined test set are very low. Whereas the scores of our mined model remain comparable on the wiki test-set in addition to maintaining a high score on its own test set. Finally the fire test set is chosen as an unbiased foreign test set where our mined model greatly outperforms.\\

\HK{table \ref{table:mbert_cross_hindi} is redundant given table \ref{table:crosstest}}.

For example for Hindi, the AI4B mined model scores 0.78, 0.60, 0.60 on the mined, WikiAnn, Fire test sets respectively. The WikiAnn model scores 0.44, 0.87, 0.39. This captures exactly what is described above. Note that such behaviour is seen on majority of the languages, but not all.

\subsection{Domain Specific Fine Tuning}
Despite the previous section, we understand that sometimes it is favourable to have models that are hyper accurate to a specific domain and are not very general. In this case it seems that training a model to a data set specific to that domain might be the way to go. \\
We carried out an experiment where a model was pre-trained to our mined data set and was then fine tuned using a small domain specific data set (WikiAnn, SE22 etc.). From this is was observed that the in-domain test scores for these data sets was actually higher using this method rather than using a model trained directly on these data sets. The improvements for each language can be seen in Table \ref{table:fine_tuning_with_AI4B_pretrain}. In addition, this pre-trained models did not loose much of their generality when tested on other domain test sets. While not as good as a model trained purely on mined data, the drop is marginal.

\subsection{Multilingual Models}
A model was trained to all the languages at once and was shown to give consistently good results across the board and the NER tasks over all languages can be handled by this one single model. This seems to be our best overall performing model. The final scores of this model on the AI4B test set and the human annotated test set can be seen in Table \ref{table:multilingual_scores}. As seen, this gives consistently high f1 scores over most languages (with the exception of As, Or).

\subsection{Next}

Compared to starting from a pre-trained model (on NLU tasks) or using a model trained in English, our mined model provides a better starting checkpoint. Training on mined data is consistently better than zero-shot results, and fine tuning this trained model on specific dataset helps to get a better score as well as can be seen from ``mined tuned on fire" and ``mined tuned on wiki" models. We can conclude that the mined dataset is of good quality, in comparison to the already present resources. 
Assamese language is a outlier in most cases since the amount of parallel sentences available between en-as is quite small when compared to any other language and most of the sentences get filtered due to absence of named entities. 

Understanding the gap in performance compared to the numbers presented by SOTA models in English - since the source of tags is the English model, which was actually trained on the CoNLL dataset, the network is more familiar with named entities of European origin. This can be a reason where the initial prediction on the Indian-English sentence is not up to the mark. Further accounting the projection errors, the quality of the mined data might not be gold standard.

This can be slightly improved using an initial model mastered in Indian English to recognize Names of Indian origin. Another place with scope for improvement is alignment. Giza++ is not the best possible way to get alignments right now, and it is slightly outdated. There are some new and better-performing models \cite{zenkel2020endtoend} for this as well. Finding and use of such models suitable for Indian languages can also help get better word to word alignment and reduce the scope for errors during projection.


\section{Conclusion}


\subsection{Training datasets to compare}

\begin{itemize}
 \item WikiAnn
 \item FIRE
 \item Sem Eval
\end{itemize}

\subsection{Transfer learning approach for comparison}

\begin{itemize}
 \item Transfer from English (train on English, evaluate on other languages)
 %The zero-shot approach~\cite{vanhoang2021zeroshot} is based on the concept of the models to understand the context behind the labels \cite{wu2019beto}. For zero-shot learning in NER, we use a network pre-trained on a set of languages. This network is fine-tuned using labeled data for a high resource language (for which a sufficiently high amount of data is available). It is assumed that the learnings can be generalized across languages. Hence, while testing or predicting, data from other languages is passed as input, and it is expected that the model can use what it has learned and predict results for this input.This technique has been found to be effective for NLP as well as CV tasks. On the upside, this does not require any additional labeled data on the target language or alignment data between languages. 
\end{itemize}

\subsection{Other baselines}

\begin{itemize}
 \item Teacher/Student based model
 %In this type of cross-lingual transfer learning, a model trained for the source language is used as a teacher model to predict the distribution of entity labels in the target language~\cite{wu2020singlemultisource}. This method does not rely on the availability of any labeled data or word alignment between sentences in a parallel corpus. This is different from zero-shot learning as the output of the teacher model is used to train a (separate) student model, which is then used as the primary model for prediction and test purposes. Experiments on Spanish, Dutch, and German using standard benchmarks were found to perform on par with state-of-the-art approaches.
 \item Struct-shot
\end{itemize}
 

\subsection{Improved models}

\begin{itemize}
 \item Joint model for All Indic languages
 \item Joint model for English+all Indic languages
 \item Above models and then finetune with language of interest
 \item Train for English, then all Indic languages and then finetune with language of interest.
\end{itemize}


\section{Related Work}
An ideal situation for such projection-based methods to work is $1$-to-$1$ alignment. However, this is not the case as sometimes a single source word would be aligned to multiple target words. Only a subset of the aligned target words would inherit the tag from the source word leaving the remaining aligned words untagged. Additionally, a target word would be generated by the \textit{null} source word. Assigning tags for such target words becomes trickier. \citet{yarowsky-ngai-2001-inducing} proposed to subscript the tag of the target words in a one-to-many alignment by their relative positions. For example, if the source word with POS tag \textit{NNP} is aligned to the target words \textit{a, b, c} then, the target word \textit{a} gets the tag \textit{NNP$_1$} followed by \textit{b} with \textit{NNP$_2$} and \textit{c} with \textit{NNP$_3$}. They later use probability estimates from $1$-to-$1$ mappings combining with probability estimates from $1$-to-$n$ mappings to assign a tag to such words.

Abstract Meaning Representation corpus which is used to train a classifier which gives initial crude tags for the named entities. The entities chosen are reinforced by the properties associated with their “Knowledge Base”. For example, if an entity has a birth-date in its “Knowledge Base”, it is mostly a person. These tags are refined using Wikipedia hyperlinks to determine the morphological boundaries of an entity.

==> sections/discussion.tex <==
\section{Analysis}
% We now present a detailed analysis of the results from our experiments.




% \subsection{Confusion Matrices}
The entity wise confusion matrices for the predictions of our mined model on Hindi and Tamil languages' test set is presented in Figure \ref{hi_conf} and \ref{ml_conf}. Here the ``B-" and ``I-" tags have been fused together for ease of presentation. 

We observe that \texttt{ORGANIZATION} tags perform the poorest compared to other entity tags. Its seen that most of the errors are in missing out entities (predicting actual tags as O). 

\begin{figure}[!htb]
 \centering
 \includegraphics[width=.5\textwidth]{Images/hi_confusion.png}
 \caption{Entity Confusion Matrix for Hindi}
 \label{hi_conf}
\end{figure}
\begin{figure}[!htb]
 \centering
 \includegraphics[width=.5\textwidth]{Images/ml_confusion.png}
 \caption{Entity Confusion Matrix for Malayalam}
 \label{ml_conf}
\end{figure}

\begin{comment}
We now present examples of few mis-classications. Consider the sentence in table \ref{hi_incorrect_tag}, ``Punjab Sarkar" which is Punjab Government should be an Organization entity. But only the ``Punjab" part of it was identified as a Location. Again in ``Kendriya Paryavaran", is not an organization and the model tags it correctly but the gold annotation is incorrect. Later on in ``Van Mantralay", the model detected only half of the entity as an organization.
\end{comment}

\begin{comment}
\begin{table}[!htb]
\centering
\resizebox{!}{0.9\columnwidth}{%
    \begin{tabular}{@{}llll@{}}
    \toprule
    \textbf{Word} & \textbf{Word Translation} & \textbf{Actual} & \textbf{Predicted} \\ \midrule
    \indicWords{84} & sultana &B-PER & B-PER \\
    \indicWords{85} & has & O & O \\
    \indicWords{86} & told & O & O \\
    \indicWords{87} & that & O & O \\
    \indicWords{88} & punjab & \textbf{B-ORG} & \textbf{B-LOC} \\
    \indicWords{89} & government & \textbf{I-ORG} & \textbf{O} \\
    \indicWords{90} & to & O & O \\
    \indicWords{91} & big & O & O \\
    \indicWords{92} & streets & O & O \\
    \indicWords{93} & projects & O & O \\
    \indicWords{94} & of & O & O \\
    \indicWords{95} & construction & O & O \\
    \indicWords{96} & work & O & O \\
    \indicWords{97} & ahead & O & O \\
    \indicWords{98} & enhance & O & O \\
    \indicWords{99} & of & O & O \\
    \indicWords{100} & for & O & O \\
    \indicWords{101} & central & \textbf{B-ORG} & \textbf{O} \\
    \indicWords{102} & environment & \textbf{I-ORG} & \textbf{O} \\
    \indicWords{103} & minister & O & O \\
    \indicWords{104} & and & O & O \\
    \indicWords{105} & forest & B-ORG & B-ORG \\
    \indicWords{106} & ministery & \textbf{I-ORG} & \textbf{O} \\
    \indicWords{107} & of & O & O \\
    \indicWords{108} & permission & O & O \\
    \indicWords{109} & got & O & O \\
    \indicWords{110} & finished & O & O \\
    \indicWords{111} & is & O & O \\
    \indicWords{112} & . & O & O \\ \bottomrule
    \end{tabular}%
}
\caption{Hindi Incorrect Prediction}
\label{hi_incorrect_tag}
\end{table}
\end{comment}
